Random quantum circuits are approximate unitary $t$-designs in depth $O\left(nt^{5+o(1)}\right)$

The applications of random quantum circuits range from quantum computing and quantum many-body systems to the physics of black holes. Many of these applications are related to the generation of quantum pseudorandomness: Random quantum circuits are known to approximate unitary $t$-designs. Unitary $t$-designs are probability distributions that mimic Haar randomness up to $t$th moments. In a seminal paper, Brand\~{a}o, Harrow and Horodecki prove that random quantum circuits on qubits in a brickwork architecture of depth $O(n t^{10.5})$ are approximate unitary $t$-designs. In this work, we revisit this argument, which lower bounds the spectral gap of moment operators for local random quantum circuits by $\Omega(n^{-1}t^{-9.5})$. We improve this lower bound to $\Omega(n^{-1}t^{-4-o(1)})$, where the $o(1)$ term goes to $0$ as $t\to\infty$. A direct consequence of this scaling is that random quantum circuits generate approximate unitary $t$-designs in depth $O(nt^{5+o(1)})$. Our techniques involve Gao's quantum union bound and the unreasonable effectiveness of the Clifford group. As an auxiliary result, we prove fast convergence to the Haar measure for random Clifford unitaries interleaved with Haar random single qubit unitaries.

==> mymath.tex <==
% ----- new thm environments ------
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{conjecture}{Conjecture}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{remark}{Remark}

%%%================================================
%%%==============  new commands  =======================
%%%================================================
%------- smaller space in,e.g., $\exp\left(x\right)$
% \let\originalleft\left
% \let\originalright\right
% \renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
% \renewcommand{\right}{\aftergroup\egroup\originalright}
\newcommand{\myleft}{\mathopen{}\mathclose\bgroup\left}
\newcommand{\myright}{\aftergroup\egroup\right}

%%% ------ rm ---------
\newcommand{\e}{\ensuremath\mathrm{e}}
\renewcommand{\i}{\ensuremath\mathrm{i}}
\newcommand{\id}{\ensuremath\mathrm{id}}
\newcommand{\rmd}{\ensuremath\mathrm{d}}
\DeclareMathOperator{\Tr}{Tr}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecmap}{vec}
\DeclareMathOperator{\matmap}{mat}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\dist}{dist}
\newcommand{\fro}{\mathrm{F}}
\newcommand{\conv}{\operatorname{conv}}
\DeclareMathOperator{\cone}{\operatorname{cone}}
\DeclareMathOperator{\lin}{\operatorname{lin}}
\DeclareMathOperator{\Comm}{Comm}
%\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Lin}{L}
\DeclareMathOperator{\Hom}{Hom}


%Felipe's shorthand mathematical notation
\newcommand*{\mcal}{\mathcal}
\newcommand*{\mbb}{\mathbb}
\newcommand*{\mrm}{\mathrm}
\newcommand*{\included}{\xhookrightarrow{}}
\newcommand*{\includes}{\xhookleftarrow{}}
\newcommand*{\onto}{\twoheadrightarrow}
\newcommand*{\oline}{\overline}

%Felipe's symbols
\def\FF{\mathbb{F}}
\def\CC{\mathbb{C}}
\def\ZZ{\mathbb{Z}}
\def\psym{P_{\text{Sym}}}
\def\stab{\mathrm{Stab}}
\newcommand*{\frob}[1]{||#1||_\text{F}}%frobenius norm



\DeclareMathOperator{\Pos}{Pos}
\DeclareMathOperator{\CPT}{CPT}
\DeclareMathOperator{\CP}{CP}
\DeclareMathOperator{\Herm}{Herm}
\DeclareMathOperator{\HT}{HT}%hermiticity and trace preserving
\DeclareMathOperator{\TP}{TP}
%\DeclareMathOperator{\HP}{HP}
\newcommand{\Sym}{\mathrm{Sym}}
\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator{\Ad}{Ad}% Adjoint rep.: Ad_U[X] = U X U^\dagger

\DeclareMathOperator{\U}{U}%unitary group U(n)
\DeclareMathOperator{\Cl}{Cl}% Clifford group Cl(n) \subset U(n)
\renewcommand{\O}{\operatorname{O}}%orthogonal group U(n)
\DeclareMathOperator{\SU}{SU}%special unitary group SU(n)

\renewcommand{\fro}{2}
\newcommand{\utpn}{\text{\rm u,tp,0}}

\DeclareMathOperator\tr{Tr}
\DeclareMathOperator\Cliff{Cl}
\DeclareMathOperator\GL{GL}

%%% -------- Landau symbols ---------
\DeclareMathOperator{\LandauO}{\mathrm{O}}
\DeclareMathOperator{\tLandauO}{\tilde{\mathrm{O}}}
\DeclareMathOperator{\LandauOmega}{\Omega}


% %%% ------- complexity -----------
% \makeatletter 
% %from complexity.sty
% \newcommand\complexity@possiblymakesmaller[1]{#1} % default: do nothing
% \newcommand\complexity@fontcommand{\mathsf} % default: do noting
% \newcommand{\ComplexityFont}[1]{%
% {\ensuremath{\complexity@possiblymakesmaller{\complexity@fontcommand{#1}}}}%extra {} makes everyone happy.
% }
% \makeatother
% \newcommand{\NP}{\ComplexityFont{NP}}
% \newcommand{\sharpP}{\#\ComplexityFont{P}}




%%% ------ mathcal ---------
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\X}{\mc{X}}
\newcommand{\Y}{\mc{Y}}
\newcommand{\V}{\mc{V}}
\newcommand{\W}{\mc{W}}
% \newcommand{\F}{\mc{F}}
\newcommand{\K}{\mc{K}}
\newcommand{\mcM}{\mc{M}}
\newcommand{\mcL}{\mc{L}}
\newcommand{\mcR}{\mc{R}}
\renewcommand{\H}{\mc{H}}
\newcommand{\landauO}{\mc{O}}
\newcommand{\DM}{\mc{S}}
\newcommand{\meas}{\mc{M}}

%%% ------ other ----------
\newcommand{\kw}[1]{\frac{1}{#1}}
\newcommand{\tkw}[1]{\tfrac{1}{#1}}
\newcommand{\argdot}{{\,\cdot\,}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\ad}{^\dagger}%symbol for conjugate transpose
\renewcommand{\L}{\operatorname{\mathrm{L}}}%linear operators
\newcommand{\LL}{\operatorname{\mathbb{L}}}%linear maps on operators
\newcommand{\M}{\operatorname{\mathbb{L}}}
% \newcommand{\DM}{\operatorname{\mc{D}}} %density operators
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\dunion}{\,\dot{\cup}\,}


%%% ------ norms, inner product ----------
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert} %norm with variable height
\newcommand{\normn}[1]{\lVert #1 \rVert} %norm with normalsize height
\newcommand{\normb}[1]{\bigl\Vert #1 \bigr\Vert} %norm with big height
\newcommand{\normB}[1]{\Bigl\Vert #1 \Bigr\Vert} %norm with Big height
\newcommand{\snorm}[1]{\norm{#1}_\infty} %spectral norm  =  (2->2)-norm
\newcommand{\snormn}[1]{\normn{#1}_\infty}
\newcommand{\snormb}[1]{\normb{#1}_\infty}
\newcommand{\snormB}[1]{\normB{#1}_\infty}
\newcommand{\tnorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\tnormn}[1]{\normn{#1}_{1}}
\newcommand{\tnormb}[1]{\normb{#1}_{1}}
\newcommand{\TrNorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\TrNormn}[1]{\normn{#1}_{1}}
\newcommand{\TrNormb}[1]{\normb{#1}_{1}}
\newcommand{\pNorm}[1]{\norm{#1}_p} %diamond norm
\newcommand{\pNormn}[1]{\normn{#1}_p}
\newcommand{\pNormb}[1]{\normb{#1}_p}
\newcommand{\fnorm}[1]{\norm{#1}_\fro} %Frobenius norm
\newcommand{\fnormn}[1]{\normn{#1}_\fro}
\newcommand{\fnormb}[1]{\normb{#1}_\fro}
\newcommand{\fnormB}[1]{\normB{#1}_\fro}
%\newcommand{\nnorm}[1]{\norm{#1}_1} %nuclear norm
%\newcommand{\nnormn}[1]{\normn{#1}_1}
%\newcommand{\nnormb}[1]{\normb{#1}_1}
\newcommand{\dnorm}[1]{\norm{#1}_\diamond} %diamond norm
\newcommand{\dnormn}[1]{\normn{#1}_\diamond}
\newcommand{\dnormb}[1]{\normb{#1}_\diamond}
\newcommand{\cbnorm}[1]{\norm{#1}_\mathrm{cb}} %cb norm
\newcommand{\jnorm}[1]{\norm{#1}_\mysquare} % \jnorm{J(M)}=dim(V)*\dnorm{M}
\newcommand{\jnormn}[1]{\normn{#1}_\mysquare}
\newcommand{\jnormb}[1]{\normb{#1}_\mysquare}
\newcommand{\threenorm}[1]{\lvert\lvert\lvert#1\rvert\rvert\rvert} % ||| . |||
\newcommand{\lTwoNorm}[1]{\norm{#1}_{\ell_2}} %\ell_2 norm
\newcommand{\lTwonormn}[1]{\normn{#1}_{\ell_2}}
\newcommand{\lTwonormb}[1]{\normb{#1}_{\ell_2}}
\newcommand{\lqNorm}[1]{\norm{#1}_{\ell_q}} %\ell_q norm
\newcommand{\lqnormn}[1]{\normn{#1}_{\ell_q}}
\newcommand{\lqnormb}[1]{\normb{#1}_{\ell_q}}
\newcommand{\TwoNorm}[1]{\norm{#1}_{2}} % 2 norm
\newcommand{\TwoNormn}[1]{\normn{#1}_{2}}
\newcommand{\TwoNormb}[1]{\normb{#1}_{2}}

%%% ---- Kets -----
%\newcommand{\ket}[1]{\left.\left|{#1}\right.\right\rangle}
\newcommand{\ketn}[1]{| #1 \rangle}
\newcommand{\ketb}[1]{\bigl| #1 \bigr\rangle}
%\newcommand{\bra}[1]{\left.\left\langle{#1}\right.\right|}
\newcommand{\bran}[1]{\langle #1 |}
\newcommand{\brab}[1]{\bigl\langle #1 \bigr|}
%\newcommand{\braket}[2]{\left\langle #1 \middle| #2 \right\rangle}
\newcommand{\braketn}[2]{\langle #1 \middle| #2 \rangle}
%\newcommand{\ketbra}[2]{\ket{#1} \!\! \bra{#2}}
\newcommand{\ketibra}[3]{\ket{#1}_{#2} \!\! \bra{#3}}
\newcommand{\ketbran}[2]{\ketn{#1} \! \bran{#2}}
\newcommand{\ketbrab}[2]{\ketb{#1} \! \brab{#2}}
\newcommand{\sandwich}[3]
  {\left\langle  #1 \right| #2 \left| #3 \right\rangle}
\newcommand{\sandwichb}[3]
  {\bigl\langle  #1 \bigr| #2 \bigl| #3 \bigr\rangle}
  
\newcommand{\oket}[1]{\left.\left|{#1}\right.\right)}
\newcommand{\obra}[1]{\left.\left({#1}\right.\right|}
\newcommand{\obraket}[2]{\left( #1 \middle| #2 \right)}
\newcommand{\oketbra}[2]{\oket{#1} \!\! \obra{#2}}
\newcommand{\osandwich}[3]
  {\left(  #1 \right| #2 \left| #3 \right)}

%%% ------ specific to this project ----------
\renewcommand{\Pr}{\operatorname{\PP}} 
\newcommand{\Ev}{\operatorname{\EE}} %expectation value
\newcommand{\A}{\mc{A}} %measurement map
\newcommand{\ev}{e} %error vector
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\st}{\mathrm{subject\ to}}
\newcommand{\Haar}{\mathrm{Haar}}
\newcommand{\minimize}{\mathrm{minimize }}
\newcommand{\maximize}{\mathrm{maximize }}
\newcommand{\Span}[1]{\langle #1 \rangle}
\newcommand{\mysquare}{{\protect\scalebox{0.5}{$\square$}}}
\renewcommand{\r}{_{|r}}
\renewcommand{\c}{_{\neg r}}
\newcommand{\rec}{\mathrm{rec}}
\newcommand{\Toff}{\mathrm{Toff}}
\newcommand{\dep}{\mathrm{dep}}
\newcommand{\eps}{\mathrm{eps}}
\newcommand{\utp}{\text{\rm u,tp}}
\newcommand{\Favg}{F_\text{avg}}





% Commands allowing to switch-on AGF abbreviation for average gate fidelity
%\newcommand{\AGF}{average gate fidelity}
\newcommand{\AGF}{AGF}
%\newcommand{\AGFs}{average gate fidelities}
\newcommand{\AGFs}{AGFs}
%Commands for consistent notation of reconstruction errors
\newcommand{\recerror}{\ensuremath\varepsilon_{\text{\rm rec}}}
\newcommand{\recerrorTr}{\ensuremath\varepsilon}
\newcommand{\recerrorF}{\ensuremath\varepsilon_{\text{\rm F}}}


%%%%%%%% Added by Markus
%%% ------ fields/sets ---------
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\F}{\mathbb{F}}


%%% ------ text ---------
\newcommand{\ie}{i.\,e.}
\newcommand{\Ie}{I.\,e.}
\newcommand{\eg}{e.\,g.}
\newcommand{\Eg}{E.\,g.} 
%\newcommand{\one}{\mathbb{1}}

\DeclareMathOperator{\spann}{span}
\newcommand{\haar}{\mu_\mathrm{H}}


% other stuff
\def\be                 {\begin{equation}}
\def\ee                 {\end{equation}}

\def\ii          {\mathrm{i}}

\def \d            {\mathrm{d}}
\def \tri          {\triangleright}
\def \L           {\mathrm{L}}
\def \rie         {\mathrm{Rie}}



